On the Convergence of FedAvg on Non-IID Data

Federated learning enables a large amount of edge computing devices to jointly learn a model without data sharing. As a leading algorithm in this setting, Federated Averaging (\texttt{FedAvg}) runs Stochastic Gradient Descent (SGD) in parallel on a small subset of the total devices and averages the sequences only once in a while. Despite its simplicity, it lacks theoretical guarantees under realistic settings. In this paper, we analyze the convergence of \texttt{FedAvg} on non-iid data and establish a convergence rate of $\mathcal{O}(\frac{1}{T})$ for strongly convex and smooth problems, where $T$ is the number of SGDs. Importantly, our bound demonstrates a trade-off between communication-efficiency and convergence rate. As user devices may be disconnected from the server, we relax the assumption of full device participation to partial device participation and study different averaging schemes; low device participation rate can be achieved without severely slowing down the learning. Our results indicate that heterogeneity of data slows down the convergence, which matches empirical observations. Furthermore, we provide a necessary condition for \texttt{FedAvg} on non-iid data: the learning rate $\eta$ must decay, even if full-gradient is used; otherwise, the solution will be $\Omega (\eta)$ away from the optimal.

==> tex/new_proof.tex <==

\section{New proof}

\subsection{Additional Notation}

Let $\w_t^k$ be the model parameter maintained in the $k$-th device at the $t$-th step. Let $\IM $ be the set of global synchronization steps, i.e., $\IM_E = \{nE \  | \ n=1,2,\cdots\}$. If $t+1 \in \IM_E$, i.e., the time step to communication, \texttt{FedAvg} randomly activates a subset of devices with the probability $p_k$. We denote by $\HM_t$ the multiset selected which is only well defined for $t \in \IM$. For convenience, we denote by $\SM_t = \HM_{N(t, E)}$ where $N(t, E) = \max\{n| n \le t, n \in \IM_E\}$. Then the update of \texttt{FedAvg} with partial devices active can be described as
\begin{align}
& \v_{t+1}^k = \w_t^k - \eta_t \nabla F_k(\w_t^k, \xi_t^k), 
\label{eq:partial_update_before}\\
& \w_{t+1}^k =\left\{\begin{array}{ll}
\v_{t+1}^k           & \text{ if } t+1 \notin \IM_E, \\
 \frac{1}{K}\sum_{k \in \SM_t}\v_{t+1}^k   & \text{ if } t+1  \in \IM_E.
 \label{eq:partial_update_after}
\end{array}\right. 
\end{align}
Here, an additional variable $\v_{t+1}^k$ is introduced to represent the immediate result of one step SGD update from $\w_t^k$. 

We define a virtual sequence $\overline{\v}_{t+1} = \frac{1}{K}\sum_{k \in \SM_t}\v_{t+1}^k$, the sample mean of updated parameters which are maintained in activated devices. Note that $\overline{\v}_{t+1}$ is inaccessible when $t+1 \in \IM_E$. When $t+1 \in \IM_E$, for all activated devices $k \in \HM_{t+1}$, $\w_{t+1}^k = \overline{\v}_{t+1}$ and hence $\overline{\w}_{t+1}=\overline{\v}_{t+1}$. 

In our analysis, there are two sources of randomness. One results from the stochastic gradients and the other is from the random sampling of devices. When we take expectation, we should distinguish them. To that end, we denote by $\EB_{\GM}(\cdot)$ the former type and $\EB_{\SM_t}(\cdot)$ the latter. 

Further, we define $\overline{\g}_t = \frac{1}{K}\sum_{k \in \SM_t} \nabla F_k(\w_t^k)$ and $\g_t = \frac{1}{K}\sum_{k \in \SM_t} \nabla F_k(\w_t^k, \xi_t^k)$. Then $\overline{\v}_{t+1} = \overline{\w}_t - \eta_t \g_t$ and $\EB_{\GM} \g_t = \overline{\g}_t$.


\subsection{Key Lemmas}
To convey our proof clearly, it would be necessary to prove certain useful lemmas. We defer the proof of these lemmas to latter section and focus on proving the main theorem.

\begin{lem}[Results of one step SGD]
\label{lem:partial_main_lem1} Assume Assumption~\ref{asm:smooth} and~\ref{asm:strong_cvx}. If $\eta_t\leq \frac{1}{4L}$, then conditioning on $\SM_t$, we have
\begin{align*}
\EB_{\GM} \left\|\av_{t+1}-\w^{\star}\right\|^{2} 
&\leq (1-\eta_t \mu) \EB_{\GM} \left\|\overline{\w}_{t}-\w^{\star}\right\|^{2} + 
\frac{2}{K} \sumk \EB_{\GM}  \| \overline{\w}_t - \w_t^k\|_2^2 +
 \eta_{t}^{2} \EB_{\GM} \left\|\mathbf{g}_{t}-\overline{\mathbf{g}}_{t}\right\|^{2}.
\\
& \quad
+ \frac{2\eta_t}{K} \sumk \left( F^* -F_k^* \right) 
+ \frac{2\eta_t}{K}\sumk \left(F_k(\w^*) - F^*\right)
\end{align*}
\end{lem}


\begin{lem}[Bounding the variance]
Assume Assumption~\ref{asm:sgd_var} holds and condition on $\SM_t$. It follows that
	\label{lem:partial_var}
	\[
	\EB_{\GM} \left\|\mathbf{g}_{t}-\overline{\mathbf{g}}_{t}\right\|^{2} 
	\leq \frac{\sumk \sigma_k^2}{K^2}.
	\]
\end{lem}


\begin{lem}[Bounding the divergence of $\{\w_t^k\}$]
	\label{lem:partial_diversity}
	Assume Assumption~\ref{asm:sgd_norm}, that $\eta_t$ is non-increasing and $\eta_{t+E} \leq 2 \eta_t$ for all $t\geq 0$. Then conditioning on $\SM_t$, we have
	\[
	\EB_{\GM} 
	\left[\frac{1}{K} \sumk \left\|\overline{\w}_{t}-\w_{k}^{t}\right\|^{2} \right]
	\: \leq \: 4 \eta_t^2 (E-1)^2 G^2.
	\]
\end{lem}


\begin{lem}
\label{lem:partial_main_lem2}
If $\eta_t\leq \frac{1}{4L}$,  we have
\begin{equation*}
\EB \left\|\av_{t+1}-\w^{\star}\right\|^{2} 
\leq (1-\eta_t \mu) \EB \left\|\overline{\w}_{t}-\w^{\star}\right\|^{2} 
+ \eta_t^2 B
\end{equation*}
where the expectation is taken for all randomness and 
\[ B =  8L\myave \left( F^* -F_k^* \right) + \frac{\myave \sigma_k^2}{K} + 8(E-1)^2 G^2.\]
\end{lem}

\begin{proof}[Proof of ]
No matter $t+1 \in \IM_E$ or $t+1 \notin \IM_E$, we always have $\aw_{t+1}= \av_{t+1}$. Let $\Delta_t=\EB \left\|\aw_{t+1}-\w^{\star}\right\|^{2}$. For a diminishing stepsize, $\eta_t = \frac{\beta}{t + \gamma}$ for some $\beta > \frac{1}{\mu}$ and $\gamma > 0$ such that $\eta_1 \le \min\{\frac{1}{\mu}, \frac{1}{4L}\}$. We prove $\Delta_t \le \frac{v}{\gamma + t}$ where $v = \max\left\{ \frac{\beta^2 B}{\beta \mu -1}, (\gamma+1)\Delta_1 \right\}$.

We prove it by induction. Firstly, the definition of $v$ ensures that it holds for $t = 1$. Assume the conclusion holds for some $t$, it follows that
\begin{align*}
\Delta_{t+1} 
&\le (1-\eta_t\mu )\Delta_t + \eta_t^2 B \\
&=\left(1- \frac{\beta\mu}{t + \gamma}\right)\frac{v}{t + \gamma} + \frac{\beta^2B}{(t + \gamma)^2}\\
&=\frac{t + \gamma -1}{(t + \gamma)^2} v  + \left[ \frac{\beta^2B}{(t + \gamma)^2} - \frac{\beta\mu-1}{(t+\gamma)^2}v \right] \\
& \le \frac{v}{t + \gamma +1}.
\end{align*}

Then by the strong convexity of $F(\cdot)$,
\[  F(\aw_t) - F^* \le \frac{L}{2} \Delta_t  \le \frac{L}{2} \frac{v}{\gamma + t}.\]
\end{proof}



\subsection{Deferred proofs of key lemmas}
\begin{proof}[Proof of Lemma~\ref{lem:partial_main_lem1}.]
	Notice that $\av_{t+1} = \aw_t - \eta_t \vg_t$, then
	\begin{align}
	\label{eq:partial_main}
	\left\|\overline{\v}_{t+1}-\w^{\star}\right\|^{2} \nonumber 
	&=\left\|\overline{\w}_{t}-\eta_{t} \mathbf{g}_{t}-\w^{\star}-\eta_{t} \overline{\mathbf{g}}_{t}+\eta_{t} \overline{\mathbf{g}}_{t}\right\|^{2} \nonumber \\ 
	&=\underbrace{\left\|\overline{\w}_{t}-\w^{\star}-\eta_{t} \overline{\mathbf{g}}_{t}\right\|^{2}}_{A_1}+
	\underbrace{2\eta_{t}\left\langle\overline{\w}_{t}-\w^{\star}-\eta_{t} \overline{\mathbf{g}}_{t}, \overline{\mathbf{g}}_{t}-\mathbf{g}_{t}\right\rangle}_{A_2} +
	\eta_{t}^{2}\left\|\mathbf{g}_{t}-\overline{\mathbf{g}}_{t}\right\|^{2}
	\end{align}
	Note that $\EB_{\GM} A_2 = 0$. We next focus on bounding $A_1$. Again we split $A_1$ into three terms:
	\begin{equation}
	\label{eq:partial_proof_main_term}
	\left\|\overline{\w}_{t}-\w^{\star}-\eta_{t} \overline{\mathbf{g}}_{t}\right\|^{2} =\left\|\overline{\w}_{t}-\w^{\star}\right\|^{2}
	\underbrace{-2 \eta_{t}\left\langle\overline{\w}_{t}-\w^{\star}, \overline{\mathbf{g}}_{t}\right\rangle}_{B_1}
	+  \underbrace{\eta_{t}^{2}\left\|\overline{\mathbf{g}}_{t}\right\|^{2}}_{B_2}
	\end{equation}
	
	From the the $L$-smoothness of $F_k(\cdot)$, it follows that
	\begin{equation}
	\label{eq:partial_proof_L}
	  \left\|\nabla F_k\left(\w_{t}^{k}\right)\right\|^{2} \leq 2 L\left(F_k\left(\w_{t}^{k}\right)-F_k^{\star}\right).
	\end{equation}
	By the convexity of $\left\| \cdot \right \|^2$ and~\eqref{eq:partial_proof_L}, we have
	\[
	B_2 = \eta_{t}^{2}\left\|\overline{\mathbf{g}}_{t}\right\|^{2} 
	\leq \frac{\eta_{t}^{2}}{K}\sumk\left\|\nabla F_k\left(\w_{t}^{k}\right)\right\|^{2}
	\leq \frac{2L\eta_t^2}{K} \sumk \left( F_k(\w_t^k) - F_k^*\right).
	\]
	Note that 
	\begin{align}
	\label{eq:partial_B1}
	  B_1 
	  &= -2 \eta_{t}\left\langle\overline{\w}_{t}-\w^{\star}, \overline{\mathbf{g}}_{t}\right\rangle 
	  = -\frac{2\eta_t}{K} \sumk \left\langle\overline{\w}_{t}-\w^{\star}, \nabla F_k(\w_t^k)\right\rangle \nonumber \\
	  &=-\frac{2\eta_t}{K} \sumk \left\langle\overline{\w}_{t}-\w_t^k, \nabla F_k(\w_t^k)\right\rangle
	  -\frac{2\eta_t}{K} \sumk \left\langle\w_t^k-\w^{\star}, \nabla F_k(\w_t^k)\right\rangle.
	\end{align}
	By Cauchy-Schwarz inequality and AM-GM inequality, we have
	\begin{equation}
	\label{eq:partial_B11}
	-2 \left\langle\overline{\w}_{t}-\w_t^{k}, \nabla F_k \left(\w_{t}^{k}\right)\right\rangle \leq \frac{1}{\eta_t} \left\|\overline{\w}_{t}-\w_{t}^{k}\right\|^{2}
	+ \eta_t \left\|\nabla F_k\left(\w_{t}^{k}\right)\right\|^{2}.	
	\end{equation}
	By the $\mu$-strong convexity of $F_k(\cdot)$, we have
	\begin{equation}
	\label{eq:partial_B12}
	-\left\langle\w_{t}^{k}-\w^{\star}, \nabla F_k\left(\w_{t}^{k}\right)\right\rangle \leq -\left(F_k\left(\w_{t}^{k}\right)-F_k(\w^*)\right)-\frac{\mu}{2}\left\|\w_{t}^{k}-\w^{\star}\right\|^{2}.
	\end{equation}
	By combining ~\eqref{eq:partial_proof_main_term},~\eqref{eq:partial_B1},~\eqref{eq:partial_B11} and~\eqref{eq:partial_B12}, it follows that
	\begin{align*}
	 A_1 
	 =  \left\|\overline{\w}_{t}-\w^{\star}-\eta_{t} \overline{\mathbf{g}}_{t}\right\|^{2} 
	 &\leq \left\|\overline{\w}_{t}-\w^{\star}\right\|^{2} 
	 + \frac{2L\eta_t^2}{K} \sumk \left( F_k(\w_t^k) - F_k^*\right) \\
	 & \quad + \frac{\eta_t }{K}\sumk \left(\frac{1}{\eta_t} \left\|\overline{\w}_{t}-\w_{k}^{t}\right\|^{2}+\eta_t \left\|\nabla F_k\left(\w_{t}^{k}\right)\right\|^{2}\right)  \\ 
	&  \quad - \frac{2\eta_t}{K} \sumk \left( \left(F_k\left(\w_{t}^{k}\right)-F_k(\w^*)\right) + \frac{\mu}{2}\left\|\w_{t}^{k}-\w^{\star}\right\|^{2} \right) \\
	& = (1-\mu\eta_t)\left\|\overline{\w}_{t}-\w^{\star}\right\|^{2} 
	+ \frac{1}{K} \sumk \left\|\overline{\w}_{t}-\w_{k}^{t}\right\|^{2} \\
	& \quad + \underbrace{	\frac{4L\eta_t^2}{K} \sumk \left( F_k(\w_t^k) - F_k^*\right) 
	 - \frac{2\eta_t}{K} \sumk  \left(F_k\left(\w_{t}^{k}\right)-F_k(\w^*)\right)}_{C}
	\end{align*}
	where we use~\eqref{eq:partial_proof_L} again.
	
	We next aim to bound $C$. We define $\gamma_t = 2\eta_t(1-2L\eta_t)$. Since $\eta_t \leq \frac{1}{4L}$, $\eta_t \le \gamma_t \leq 2\eta_t$. Then we split $C$ into three terms:
	\begin{align*}
	 C &= - \frac{2\eta_t(1-2L\eta_t)}{K} \sumk \left( F_k(\w_t^k) - F_k^* \right) 
	 + \frac{2\eta_t}{K}\sumk \left(F_k(\w^*) - F_k^*\right) \\
	 &=-\frac{\gamma_t}{K}\sumk \left( F_k(\w_t^k) - F^* \right)  
	 -\frac{\gamma_t}{K}\sumk \left( F^*-F_k^*\right)  
	+ \frac{2\eta_t}{K}\sumk \left(F_k(\w^*) - F_k^*\right) \\
	 &=-\underbrace{\frac{\gamma_t}{K}\sumk \left( F_k(\w_t^k) - F^* \right)}_{D}
	 +\frac{4L\eta_t^2}{K}\sumk \left( F^*-F_k^*\right)  
	 + \frac{2\eta_t}{K}\sumk \left(F_k(\w^*) - F^*\right)
	\end{align*}
	To bound $D$, we have
	\begin{align*}
 \frac{1}{K} \sumk \left( F_k(\w_t^k) - F^*  \right)
	 &=\frac{1}{K} \sumk \left( F_k(\w_t^k) - F_k(\overline{\w}_t)  \right) 
	 + \frac{1}{K} \sumk \left( F_k(\overline{\w}_t) - F^*  \right)\\
	 & \ge \frac{1}{K} \sumk\left\langle \nabla F_k(\overline{\w}_t), \overline{\w}_t^k - \overline{\w}_t \right\rangle
	 + \frac{1}{K} \sumk \left( F_k(\overline{\w}) - F^*  \right)\\
	 & \ge - \frac{1}{2K}\sumk \left[ \eta_t\left\|  \nabla F_k(\overline{\w}_t) \right\|^2 + \frac{1}{\eta_t}\left\|\w_t^k -\overline{\w}_t\right\|^2 \right]
	 + \frac{1}{K} \sumk \left( F_k(\overline{\w}_t) - F^*  \right)\\
	 & \ge - \frac{1}{K}\sumk \left[ \eta_tL \left(F_k(\overline{\w}_t) -F_k^*   \right)
	 + \frac{1}{2\eta_t}\left\|\w_t^k -\overline{\w}_t\right\|^2 \right]
	 + \frac{1}{K} \sumk \left( F_k(\overline{\w}_t) - F^*  \right)
	\end{align*}
	where the first inequality results from the convexity of $F_k(\cdot)$, the second inequality from AM-GM inequality and the third inequality from~\eqref{eq:partial_proof_L}.
	
	Therefore 
	\begin{align*}
	  C 
	  &= \frac{\gamma_t}{K}\sumk \left[ \eta_tL \left(F_k(\overline{\w}_t) -F_k^*   \right)
	 + \frac{1}{2\eta_t}\left\|\w_t^k -\overline{\w}_t\right\|^2 \right]
	 - \frac{\gamma_t}{K} \sumk \left( F_k(\overline{\w}_t) - F^*  \right) \\
	 & \quad +\frac{4L\eta_t^2}{K}\sumk \left( F^*-F_k^*\right)  
	 + \frac{2\eta_t}{K}\sumk \left(F_k(\w^*) - F^*\right)\\
	 &= \frac{\gamma_t}{K}(\eta_t L -1 ) \sumk \left(F_k(\aw_t) -F_k^* \right)
	 + \frac{4L\eta_t^2 + \gamma_t}{K} \sumk \left( F^* - F_k^*\right) \\
	 & \quad + \frac{\gamma_t}{2\eta_t K} \sumk \left\|\w_t^k -\overline{\w}_t\right\|^2 
	 + \frac{2\eta_t}{K} \sumk \sumk \left(F_k(\w^*) - F^*\right)\\
	 &\le \frac{4L\eta_t^2}{K} \sumk \left( F^* - F_k^*\right)
	 + \frac{1}{K} \sumk \left\|\w_t^k -\overline{\w}_t\right\|^2 
	 + \frac{2\eta_t}{K} \sumk \left(F_k(\w^*) - F^*\right)
	\end{align*}
	where in the last inequality, we use the following facts: (1) $\eta_t L -1 \le - \frac{3}{4} \le 0$ and  $F_k(\aw_t) -F_k^*\ge 0$ and (2) $\frac{\gamma_t}{2\eta_t} \le 1$.
	
	Recalling the expression of $A_1$ and plugging $C$ into it, we have
	\begin{align}
	\label{eq:partial_proof_A1}
	  A_1 
	  &= \left\|\overline{\w}_{t}-\w^{\star}-\eta_{t} \overline{\mathbf{g}}_{t}\right\|^{2} \nonumber\\
      &\le (1-\mu\eta_t)\left\|\overline{\w}_{t}-\w^{\star}\right\|^{2} 
	  + \frac{2}{K} \sumk \left\|\overline{\w}_{t}-\w_{k}^{t}\right\|^{2} \nonumber \\
	  & \quad + \frac{1}{K} \sumk \left\|\w_t^k -\overline{\w}_t\right\|^2 
	 + \frac{2\eta_t}{K} \sumk \left(F_k(\w^*) - F^*\right)
	\end{align}
	Using~\eqref{eq:partial_proof_A1} and taking expectation on both sides of~\eqref{eq:partial_main}, we erase the randomness from stochastic gradients, we complete the proof.
\end{proof}



\begin{proof}[Proof of Lemma~\ref{lem:partial_var}]
    From Assumption~\ref{asm:sgd_var}, the variance of the stochastic gradients in device $k$ is bounded by $\sigma_k^2$, then
	\begin{align*}
	\EB_{\GM} \left\|\mathbf{g}_{t}-\overline{\mathbf{g}}_{t}\right\|^{2}  
	& = \EB \left\|\frac{1}{K} \sumk (\nabla F_k(\w_t^k,\xi_t^k) - \nabla F_k(\w_t^k))  \right\|^{2} \\
	&= \sumk \frac{1}{K^2} 
	\EB \left\|  \nabla F_k(\w_t^k,\xi_t^k) - \nabla F_k(\w_t^k)  \right\|^{2} \\
	& \leq \frac{1}{K^2} \sumk \sigma_k^2.
	\end{align*}
\end{proof}



\begin{proof}[Proof of Lemma~\ref{lem:partial_diversity}]
    Since \texttt{FedAvg} requires a communication each $E$ steps. Therefore, for any $t \ge 0$, there exists a $t_0 \leq t$, such that $t-t_0 \leq E-1$ and $\w_{t_0}^k=\aw_{t_0}$ for all $k=1,2,\cdots,N$. Also, we use the fact that $\eta_t$ is non-increasing and $\eta_{t_0} \leq 2 \eta_t$ for all $t-t_0 \leq E-1$, then
	\begin{align*}
	 \EB_{\GM} \sumk \frac{1}{K} \left\|\overline{\w}_{t}-\w_{k}^{t}\right\|^{2} 
	 &= \EB_{\GM} \frac{1}{K} \sumk \left\|  (\w_{k}^{t} - \aw_{t_0})  - (\overline{\w}_{t} - \aw_{t_0})   \right\|^{2} \\
	&\leq\EB_{\GM}  \sumk \frac{1}{K} \left\|  \w_{k}^{t} - \aw_{t_0}  \right\|^{2} \\
	& \leq \sumk \frac{1}{K} \EB_{\GM} \sum_{t = t_0}^{t-1}(E-1) \eta_t^2 \left\|  \nabla F_k(\w_k^{t},\xi_k^t)     \right\|^2 \\
	& \leq \sumk \frac{1}{K}\sum_{t=t_0} ^{t-1} (E-1) \eta_{t_0}^2 G^2 \\
	& \leq \sumk \frac{1}{K}  \eta_{t_0}^2 (E-1)^2 G^2 \\
	& \leq 4 \eta_t^2 (E-1)^2 G^2.
	\end{align*}
\end{proof}


\begin{proof}[Proof of Lemma~\ref{lem:partial_main_lem2}]
We first give a key observation which is useful to prove the followings. Let $\{x_i\}_{i=1}^N$ denote any fixed deterministic sequence. We sample a multiset $\SM_t$ (with size $K$) in an i.i.d. fashion with some probability $p_k$. Let $\SM_t = \{Y_1, \cdots, Y_K\} \subset [N]$ (some $Y_k$'s may have the same value but they are sampled independently). Then
\[  \EB_{\SM_t}  \sumk x_k = \EB_{\SM_t}  \sum_{k=1}^K x_{Y_k} = K \EB_{\SM_t}  x_{Y_1} = K\myave x_k. \]
Equipped with this observation, from Lemma~\ref{lem:conv_variance}, we have
\[ \EB \left\|\mathbf{g}_{t}-\overline{\mathbf{g}}_{t}\right\|^{2} 
= \EB_{\SM_t} \EB_{\GM} \left\|\mathbf{g}_{t}-\overline{\mathbf{g}}_{t}\right\|^{2}   
\le \EB_{\SM_t} \frac{1}{K^2} \sumk \sigma_k^2 = \frac{\myave \sigma_k^2}{K}. \]
From Lemma~\ref{lem:partial_diversity}, we have
\[ \EB \sumk \frac{1}{K} \left\|\overline{\w}_{t}-\w_{k}^{t}\right\|^{2}  
= \EB_{\SM_t} \EB_{\GM} \sumk \frac{1}{K} \left\|\overline{\w}_{t}-\w_{k}^{t}\right\|^{2}
\le 4 \eta_t^2 (E-1)^2 G^2.   \]
Similarly, it follows that $\EB_{\SM_t} \frac{1}{K}\sumk \left(F_k(\w^*) - F^*\right) = \myave \left(F_k(\w^*) - F^*\right) = 0$ and
\[  \EB_{\SM_t} \frac{1}{K} \sumk \left( F^* - F_k^* \right) =\myave \left(F^* -F_k^* \right) = \Gamma. \]

Combine this results and recall Lemma~\ref{lem:partial_main_lem1}. Then we finish the proof.
\end{proof}
